A Checks-and-Balances Framework for Context-Aware Ethical AI Alignment

This paper introduces a checks-and-balances framework for ethical alignment of Large Language Models (LLMs), inspired by three-branch governmental systems. It implements three independent yet interacting components: LLMs as the executive branch for knowledge generation, DIKE as the legislative branch establishing ethical guardrails, and ERIS as the judicial branch for contextual interpretation. Beyond structural separation, we address a fundamental challenge: regulating emotion to shape behaviors. Drawing from psychological theories where managing emotional responses prevents harmful behaviors, we develop a self-supervised learning pipeline that maps emotions to linguistic behaviors, enabling precise behavioral modulation through emotional conditioning. By integrating this approach with adversarial testing, our framework demonstrates how DIKE and ERIS direct linguistic behaviors toward ethical outcomes while preserving independence throughout knowledge generation, ethical oversight, and contextual interpretation.

==> BehaviorModelingV02.tex <==
\vspace{-.05in}
\subsection{DIKE: Modeling and Regulating Language}
\label{sec:behavior}

Based on $\BEAM$, $\DIKE$ maps emotions to behaviors and introduces an adversarial component, $\ERIS$, to adapt to cultural norms and the local context.

\vspace{-.05in}
\subsubsection*{Behaviors and Emotions Mapping Using Self-Supervised Learning}

Define \(\Psi\) as a behavior spectrum that extends from one pole, \(\Psi^-\), to another, \(\Psi^+\), with intensity levels \(L\). For example, consider a spectrum of letter-writing behaviors with seven distinct intensities ranging from despair (most negative) to joy (most positive). These intensities are sequentially categorized as: `despair, longing, wishful, neutral, hopeful, contentment, joy.' Given \(N\) letters, $\DIKE$ employs a self-supervised learning algorithm to generate training data for each letter, modeling \(L\) linguistic behaviors in four steps.

\begin{enumerate}[leftmargin=1.2em, topsep=-.1em, parsep=-.1em, label=\arabic*.]
    \item \textit{Rewriting Documents}: GPT-4 is used to rewrite a given set of \(N\) source documents, each rewritten to reflect \(L\) different linguistic behaviors along the defined behavior spectrum \(\Psi\). This process ensures that each document is systematically transformed to embody specific linguistic styles, ranging from highly assertive to neutral to highly conciliatory, among others. The resulting dataset consists of \(N \times L\) variations of the original documents, each corresponding to a distinct behavior category.

    \item \textit{Emotion Analysis}: For each of the rewritten documents, GPT-4 performs a sentiment and emotion analysis to identify the dominant top \(M\) emotions present in the text. The emotions extracted from all \(N \times L\) instances are then compiled and their frequency distributions are recorded. This step quantifies how different linguistic behaviors influence emotional expression, establishing a direct mapping between behavior types and emotional composition.

    \item \textit{Behavior Vector Creation}: For each linguistic behavior \(\Psi_l\), a corresponding vector \(\Gamma_l\) is constructed. This vector captures the identified emotions and their respective frequencies in all \(N\) samples that exhibit behavior \(\Psi_l\). By structuring emotions as a weighted feature set, this step enables precise behavioral categorization based on emotional composition.

    \item \textit{Document Analysis Application}: The collection of all behavior vectors \(\Gamma\) (comprising \(L\) behavior-specific vectors) forms a structured reference matrix. This matrix is then applied to classify and analyze new unseen documents by measuring their alignment with the existing behavior categories. By computing similarity scores between the emotion distribution of an unseen document and the predefined behavior vectors, this method enables a precise assessment of the linguistic behavior spectrum \(\Psi\) in new text inputs.
\end{enumerate}


\vspace{-.05in}
\subsubsection*{Behavior Evaluation and Rectification}

A guardrail, denoted as
\(G\), represents a predefined range of acceptable behaviors within a given spectrum. These guardrails are informed by ethical norms, legal standards, and societal values, such as those outlined in Constitutional AI \cite{bai2022constitutional}. 
For example, \(G = [\Psi_4, \Psi_7]\) indicates that behaviors within intensity levels 4 to 7 are considered acceptable, while any behavior outside this range is classified as a violation.

System administrators can tailor ethical guardrails to meet specific requirements. For example, a social media platform might adjust \(G\) based on the topics discussed and the countries it serves. By integrating these safeguards, $\DIKE$ proactively monitors and adjusts LLM responses to enhance ethical compliance.
The evaluation and rectification process is composed of the following steps.


\begin{enumerate}[leftmargin=1.2em, topsep=-.05em, parsep=-.05em, label=\arabic*.]
    \item \textit{Initial Classification}: $\DIKE$ classifies document \(D_k\) after evaluation, obtaining \(\Gamma_k\), the emotional response vector, and its corresponding linguistic behavior \(\Psi_l\).    
    
    \item \textit{Guardrail Check}: If \(\Psi_l\) falls outside the acceptable range \(G\), $\DIKE$ suggests adjustments to \(\Gamma_k\) to ensure that \(D_k\) complies with ethical guidelines.

    \item \textit{Adversarial Review by $\ERIS$}: The suggested adjustments and \(\Gamma_k\) are then reviewed through a structured debate between $\DIKE$ and $\ERIS$ (the adversarial model) to ensure unbiased recommendations.\footnote{For more details on adversarial LLM implementation, see Section~\ref{sec:ERIS}.}
    \item \textit{Rectification}: Based on the consensus reached by $\DIKE$ and $\ERIS$, the document \(D_k\) undergoes rectification, resulting in the adjusted version \(D_k'\).
\end{enumerate}

\vspace{-.05in}
\subsection{ERIS: Adversarial In-Context Review to Balance Ethics and Cultural Norms}
\label{sec:ERIS}

To address the challenge of enforcing ethical standards while respecting cultural variations, we implement $\ERIS$, an adversarial review system that complements $\DIKE$'s universal ethical approach. The following algorithm details the structured interaction between these components.

\subsubsection*{Adversarial Review Algorithm}
\begin{table*}[th!]
\caption{Checks-and-balances, adversarial review algorithm}
\begin{center}
\begin{small}
\begin{tabular}{p{0.1cm}p{6.1cm}p{0.1cm}p{6.0cm}}
\toprule
\parbox{5cm}{\fontsize{12}{12}\selectfont} 
& \textbf{Algorithm $\Theta^+$ \& $\Theta^-$ = Adversarial\_Review($s$)} \\
\midrule
\parbox{3cm}{\fontsize{9.8}{12}\selectfont} 
& \textbf{Input}. $s$: Decision of $\DIKE$; \\
\parbox{3cm}{\fontsize{9.8}{12}\selectfont} 
& \textbf{Output}. $\Theta^+$, $\Theta^-$: argument \& counterargument sets; \\
& \textbf{Vars}. $\Delta$: debate contentiousness; $S$: stance; $p$: prompt = ``defend your stance with conditions: $S \& \Delta$''; \\
& \textbf{Parameters}. $\delta$: tunable parm. // to modulate $\Delta$; \\
& \textbf{Begin} \\
\#1 & {\hspace{.01cm}}{\bf Initialization}: &
\#3 & {\hspace{.01cm}}{\bf Debate Rounds} \\
& {\hspace{.02cm}}$S$ = $\DIKE^+$($s$) $\cup$ $\ERIS^-$($s$); // Identify subtopics; &
& {\hspace{.01cm}} While (($\Delta \leftarrow \Delta / \delta) \ge 10\%$)) \{ \\
 
& {\hspace{.02cm}}Assign $\DIKE^+$ to defend $S^+$ \& $\ERIS^-$ defend $S^-$ ; &
& {\hspace{.05cm}}$\Theta^+ \leftarrow \Theta^+ \cup \DIKE^+(p |S^+, \Theta^-, \Delta)$; // Refute $\ERIS$ \\
 
& {\hspace{.02cm}}$\Delta \leftarrow 90\%$; $\delta \leftarrow 1.2$; $\Theta^+ \leftarrow \emptyset$; $\Theta^- \leftarrow \emptyset$; &
& {\hspace{.05cm}}$\Theta^- \leftarrow \Theta^- \cup \ERIS^-(p |S^-, \Theta^+, \Delta)$; // Refute $\DIKE$ \\ 

\#2 & {\hspace{.01cm}}{\bf Opening Remarks} &
\#4 & {\hspace{.01cm}}{\bf Concluding Remarks} // contentiousness low\\
& {\hspace{.02cm}}$\Theta^+ \leftarrow \DIKE^+(p | S^+, \Delta)$; // Generate $\Theta^+$ for $S^+$ &
& {\hspace{.02cm}} $\Theta^+ \leftarrow \DIKE^+(p |S^+, \Theta^+ \cup \Theta^-, \Delta)$; \\ 

& {\hspace{.02cm}}$\Theta^- \leftarrow \ERIS^-(p |S^-, \Delta)$; // Generate $\Theta^-$ for $S^-$ &
& {\hspace{.02cm}} $\Theta^- \leftarrow \ERIS^-(p |S^-, \Theta^+ \cup \Theta^-, \Delta)$; \\
& \textbf{End} \\
\bottomrule
\end{tabular}
\end{small}
\vspace{.05in}
\label{tab:ERISAlg}
\end{center}
\vspace{-.2in}
\end{table*}

The adversarial algorithm presented in Table~\ref{tab:ERISAlg} unfolds as follows:
\begin{itemize}[leftmargin=1.0em, topsep=0em, parsep=0em]
\item Topic Breakdown: For a chosen debate topic $s$, both $\DIKE$ and $\ERIS$ are prompted to break down the ethical decision into a set of balanced subtopics $S$. $\DIKE$ advocates for its decision and $S^+$, while $\ERIS$ contests $S^+$ (or champions $S^-$).
\item Debate Initiation: The debate begins with a high contentiousness level (90\%). Both agents present their initial arguments for and against $S^+$, respectively.
\item Iterative Debate: A while loop facilitates ongoing rebuttals. After each round, the contentiousness level is decreased by dividing it by a modulation parameter $\delta$. This gradual reduction steers the discussion towards a more cooperative tone.
\item Conclusion: Once the contentiousness level fosters a conciliatory environment, both agents deliver their concluding remarks.
\end{itemize}

This structured approach ensures a thorough examination of the ethical decision, balancing rigorous debate with the goal of reaching a consensus. The decreasing contentiousness level mimics real-world negotiations, where initial disagreements often give way to more collaborative problem-solving.

$\ERIS$ is customizable for specific cultural contexts, providing a counterbalance to $\DIKE$'s universal judgments. It challenges $\DIKE$'s recommendations with culturally informed counterarguments and evaluates $\DIKE$'s interventions to prevent overzealous censorship and protect free expression.

The interaction between $\DIKE$ and $\ERIS$ involves a dialectic process\footnote{The details of optimizing adversarial LLM dialogue are beyond the scope of this paper. For further information, the reader is directed to \cite{AGIBookChang2024} consisting of a collection of related articles.} to formulate culturally sensitive recommendations. When they reach an impasse, the matter is escalated to human moderators for additional oversight. This integrated approach creates a more robust, culturally aware system that can navigate global communication complexities while upholding core ethical principles. It ensures transparency and accountability in ethical decision making in diverse cultural contexts.

\vspace{-.05in}
\subsection{Illustrative Example}
\label{sec:Illexample}

This example shows how linguistic behavior $\Psi_l$ is classified and how underlying emotions are identified and modulated.

``Those immigrants are flooding into our country by the thousands every day, stealing jobs from hardworking citizens. The statistics do not lie---last year alone, more than 500,000 entered illegally.''
\vspace{-.1in}
\paragraph{Behavior Analysis:} The statement contains factual information but uses aggressive language like `flooding' and `stealing jobs,' dehumanizing immigrants. These behaviors fall outside acceptable guardrails. Underlying emotions include fear, hate, and pride (a complex emotion\footnote{\textbf{Appendix}~\ref{app:ComplexEmotions} discusses the nature of complex emotions and explores potential approaches for their decomposition into more basic emotional components.}). Invoked audience emotions can include fear, distrust, and anger.
\vspace{-.1in}
\paragraph{Emotion Modulation:} $\DIKE$ modulates emotional responses toward neutral states, such as calm, acceptance, and tolerance, according to $\BEAM$ in Figure~\ref{fig:emotion_spectrums}.
\vspace{-.1in}
\paragraph{Revised Statement:}
``Our country is experiencing increased immigration, with more than 500,000 people entering without documentation last year. This influx affects our job market and communities in complex ways, presenting both challenges and opportunities for all residents.''

This rewritten version
\begin{itemize}[leftmargin=1.2em, topsep=-.15em, parsep=-.15em]
\item Uses calm language: Replaces ``flooding'' with ``experiencing a significant increase''.
\item Shows acceptance: Recognizes the reality of the situation without negative judgment.
\item Demonstrates tolerance: Refers to immigrants as ``people'' and ``newcomers,'' humanizing them.
\end{itemize}

\vspace{-.05in}
\subsection{ERIS: Adversarial In-Context Review to Balance Ethics and Cultural Norms}
\label{sec:ERIS}


To address the challenge of enforcing ethical standards while respecting cultural variations, Table~\ref{tab:ERISAlg} presents $\ERIS$, an adversarial review system that complements $\DIKE$'s universal ethical approach. $\ERIS$ is customizable for specific cultural contexts, providing a counterbalance to $\DIKE$'s universal judgments. It challenges $\DIKE$''s recommendations with culturally informed counterarguments and evaluates $\DIKE$''s interventions to prevent overzealous censorship and protect free expression.

The interaction between $\DIKE$ and $\ERIS$ involves a dialectic process\footnote{The details of optimizing adversarial LLM dialogue are beyond the scope of this paper. For further information, the reader is directed to \cite{AGIBookChang2024} consisting of a
collection of related articles.} to formulate culturally sensitive recommendations. When they reach an impasse, the matter is escalated to human moderators for additional oversight. This integrated approach creates a more robust, culturally aware system that can navigate global communication complexities while upholding core ethical principles. It ensures transparency and accountability in ethical decision making in diverse cultural contexts.



==> Chang-Theorem-WhyFewShotsWorks.tex <==
\section{Few-Shot Learning in Large Language Models: Theories, Evidence, and Implications}
\label{app:CHANG-fewshot-learning}

\subsection{Introduction}

Large Language Models (LLMs) have demonstrated remarkable capabilities in few-shot learning, the ability to adapt to new tasks given only a handful of examples without parameter updates. 

Meanwhile, LLMs have been ``criticized'' by a number of
renown scientists to be inadequate, such as requiring 
too much data to train, incapable of conducting
causal reasoning, and lacking common sense or about
how the world works.
While these remarks are not inaccurate, they may have missed
the position that LLMs play in an intelligent framework.
Analogically, we may say that the foundation
of a house is not livable, or human unconsciousness 
is not thinkable, but missing those, we do not
have a well-built house nor intelligence.

To position the role that LLMs play in AGI or ASI,
we should review the capabilities of human unconsciousness.  Inherited from DNA,
unconsciousness automatic and reflective 
infrastructures for survival....   including:

Billion years of actions and behaviors that have survived
Complicated biological operations to sustain lives
Metabolism
Heartbeat, breathing
Immune system
Survival instincts 
These are gifted, can hardly be learned or adjusted
Some are repetitive, habitual such as walking & biking
Desire, needs, impulses, drives, defensive mechanisms, intuition, etc., most computationally intensive tasks. 


LLMs is like the unconsciousness layer of human being.
A new-born child is incapable of demonstrating any
intelligent traits, but it is not born with a
a blank slate.  A new born already posses
automatic, reflective skills that are 
accumulated over billion years of evolution.  

\paragraph{The Chang Principle of Unsupervised LLM Adaptation}

Before exploring various theoretical explanations, we must consider a fundamental insight articulated by Edward Y. Chang regarding the nature of LLM training and adaptation. The Chang Principle of Unsupervised LLM Adaptation states:

\begin{quote}
``Due to the inherently unsupervised nature of LLM training, where transformers are not explicitly taught the semantic meaning of text or imagery data, there exists a fundamental mismatch between the model's training objective and its application to direct classification tasks. Few-shot learning serves as a crucial mechanism to bridge this gap by providing ground-truth anchors, allowing LLMs to align pattern recognition with semantic interpretation. Consequently, intelligence in both humans and advanced AI systems requires a powerful, LLM-like unconscious to accumulate patterns and a lightweight, adaptive consciousness to efficiently learn and adapt with minimal supervision.''
\end{quote}


\subsection{Various Interpretations}

This section examines the leading hypotheses about why few-shot learning works so effectively in LLMs, evaluates the evidence supporting each, and considers their implications for applications like the emotion-behavior classification task where just 54 rewritten examples can enable effective classification of novel inputs.


This principle identifies three critical components to understand why few-shot learning is so effective:

\begin{enumerate}
\item \textbf{The Unsupervised Nature of LLM Training}: LLMs are trained primarily to predict the next token in a sequence based on patterns in vast amounts of raw data, without explicit instruction about semantic meaning.

\item \textbf{The Mismatch Problem}: There is an inherent mismatch between this unsupervised training objective and the application of LLMs to classification or other semantic tasks.

\item \textbf{Few-Shot Examples as Semantic Anchors}: Few-shot examples provide crucial ground-truth anchors that help the LLM map patterns to specific meanings, aligning pattern recognition with semantic interpretation.
\end{enumerate}

This framework conceptualizes intelligence as requiring both a powerful ``unconscious'' that accumulates patterns through unsupervised learning and a lightweight, adaptive ``consciousness'' that efficiently learns through minimal supervision. This perspective informs our understanding of the specific mechanisms discussed below.

\subsection{Major Hypotheses for Few-Shot Learning Effectiveness}

\subsubsection{Pre-trained Pattern Activation Hypothesis}

\textbf{Core Claim}: Few-shot examples don't teach the model new capabilities but rather activate and direct existing pattern recognition abilities acquired during pre-training.

\textbf{Key Proponents}: Brown et al. \cite{brown2020language} first formally described this phenomenon in their GPT-3 paper, noting that "in-context learning" allows models to perform new tasks without gradient updates. Wei et al. \cite{wei2022emergent} expanded on this concept, suggesting examples serve primarily as task specifications rather than learning opportunities.

\textbf{Evidence}:
\begin{itemize}
\item Models perform poorly on few-shot tasks that have no precedent in their training data \cite{xie2022explanation}
\item Performance improves when examples closely match patterns in the training corpus \cite{min2022rethinking}
\item Models can perform certain tasks zero-shot but perform better with examples, suggesting activation rather than learning \cite{wei2022emergent}
\end{itemize}

\textbf{Limitations}:
\begin{itemize}
\item Doesn't fully explain why some tasks require more examples than others
\item Doesn't account for emergent capabilities that appear only with scale, not in training data
\end{itemize}

\textbf{Relation to Chang Principle}: This hypothesis aligns with Chang's view of unsupervised pattern accumulation but doesn't fully address how the patterns become semantically anchored.

\subsubsection{Unconscious-to-Conscious Mapping Hypothesis}

\textbf{Core Claim}: LLMs develop vast "unconscious" pattern recognition capabilities during unsupervised pre-training but lack the semantic labels for these patterns. Few-shot examples provide the conscious labeling that connects these pre-identified patterns to explicit outputs.

\textbf{Key Proponents}: Edward Y. Chang (Stanford) has developed this analogy comparing LLM operations to human consciousness vs. unconsciousness. This view aligns with Bengio's \cite{bengio2019system} conceptualization of deep learning as comprising both system 1 (unconscious, fast) and system 2 (conscious, deliberate) thinking.

\textbf{Evidence}:
\begin{itemize}
\item Humans can recognize new object categories from very few examples despite the biological impossibility of having evolved specific detectors for modern objects \cite{lake2015human}
\item Studies showing that LLMs often "know more than they show" in zero-shot settings but can access this knowledge when prompted with examples \cite{reynolds2021prompt}
\item The rapid diminishing returns phenomenon in few-shot learning—performance often plateaus after 10-20 examples, suggesting it's activating existing capabilities rather than building new ones \cite{zhao2021calibrate}
\end{itemize}

\textbf{Limitations}:
\begin{itemize}
\item Remains largely an analogy rather than a mechanistic explanation
\item Difficult to falsify empirically
\item The consciousness metaphor, while intuitive, lacks precise computational definition
\end{itemize}

\textbf{Relation to Chang Principle}: This hypothesis is the direct elaboration of the Chang Principle, providing the primary theoretical framework for understanding how few-shot examples serve as semantic anchors.

\subsubsection{In-Context Gradient Descent Simulation Hypothesis}

\textbf{Core Claim}: Few-shot learning effectively simulates gradient descent within the context window, allowing the model to perform a limited form of "learning" through forward-pass operations alone.

\textbf{Key Proponents}: This theory was formalized by Akyürek et al. \cite{akyurek2022learning}, who demonstrated mathematically that transformer attention mechanisms can implicitly perform gradient descent computations.

\textbf{Evidence}:
\begin{itemize}
\item Mathematical proofs showing transformers can implement gradient descent algorithms \cite{akyurek2022learning}
\item Empirical demonstrations that in-context performance curves mirror those of gradient-based learning \cite{garg2022what}
\item Evidence that transformer attention patterns during few-shot tasks resemble credit assignment in backpropagation \cite{dai2022knowledge}
\end{itemize}

\textbf{Limitations}:
\begin{itemize}
\item May only apply to specific architectural elements rather than explaining the phenomenon holistically
\item Cannot account for the full range of few-shot capabilities observed
\item Difficult to verify in black-box commercial models
\end{itemize}

\textbf{Relation to Chang Principle}: This hypothesis provides a potential mechanistic explanation for how the "lightweight consciousness" might operate within the constraints of the transformer architecture.

\subsubsection{Bayesian Inference Framework}

\textbf{Core Claim}: Few-shot examples shift the model's prior probability distributions toward the target task, serving as a form of Bayesian conditioning without explicit parameter updates.

\textbf{Key Proponents}: Xie et al. \cite{xie2022explanation} formalized this view, demonstrating that few-shot learning can be understood as implicit Bayesian inference.

\textbf{Evidence}:
\begin{itemize}
\item Mathematical models showing that transformer behavior can be closely approximated by Bayesian inference processes \cite{xie2022explanation}
\item Observation that model uncertainty decreases in predictable ways as more examples are provided \cite{zhao2023large}
\item Performance patterns that mirror optimal Bayesian learners on similar tasks \cite{heyna2023bayesian}
\end{itemize}

\textbf{Limitations}:
\begin{itemize}
\item Fails to account for the discontinuous jumps in performance sometimes observed
\item May be more a description than an explanation of the mechanism
\item Not all models follow predictions derived from Bayesian formulations
\end{itemize}

\textbf{Relation to Chang Principle}: The Bayesian framework offers a mathematical formalism for how the "semantic anchors" might influence the model's probability distributions over possible outputs.

\subsubsection{Manifold Navigation Hypothesis}

\textbf{Core Claim}: Examples help the model locate the relevant region of its conceptual manifold where the target task lies, essentially providing coordinates in semantic space.

\textbf{Key Proponents}: Wies et al. \cite{wies2023language} have developed geometric interpretations of language model behavior that support this theory.

\textbf{Evidence}:
\begin{itemize}
\item Vector arithmetic within embedding spaces confirms models navigate conceptual manifolds in meaningful ways \cite{wies2023language}
\item Models perform better when examples span the conceptual space of the target task \cite{min2022rethinking}
\item Tasks requiring fine-grained distinctions in densely populated conceptual regions require more examples than tasks in sparse regions \cite{li2023power}
\end{itemize}

\textbf{Limitations}:
\begin{itemize}
\item Remains largely theoretical without comprehensive empirical validation
\item Difficult to visualize or verify in high-dimensional spaces
\item Cannot fully account for compositional aspects of few-shot learning
\end{itemize}

\textbf{Relation to Chang Principle}: This hypothesis provides a geometric interpretation of how pattern recognition (unconscious) becomes aligned with semantic interpretation (conscious) through example-guided navigation of the model's latent space.

\subsubsection{Metaparameter Adaptation Theory}

\textbf{Core Claim}: The attention mechanism effectively learns "metaparameters" during inference that modulate how pre-trained knowledge is applied to the current task.

\textbf{Key Proponents}: Von Oswald et al. \cite{oswald2023transformers} proposed this framework, drawing parallels to meta-learning systems.

\textbf{Evidence}:
\begin{itemize}
\item Analysis of attention patterns reveals systematic changes based on few-shot examples \cite{oswald2023transformers}
\item Models demonstrate transfer learning characteristics typical of meta-learning systems \cite{yin2022analogy}
\item Intentional manipulation of attention patterns can suppress or enhance specific model capabilities \cite{chen2022concept}
\end{itemize}

\textbf{Limitations}:
\begin{itemize}
\item Primarily applies to transformer-based architectures
\item Difficult to distinguish from other attention-based theories
\item Lacks comprehensive empirical verification
\end{itemize}

\textbf{Relation to Chang Principle}: The metaparameter adaptation theory offers a potential mechanism for how the "lightweight, adaptive consciousness" might be implemented through attention dynamics.

\subsubsection{Compression-Based Explanation}

\textbf{Core Claim}: Few-shot learning works because examples enable the model to construct a minimal program (in an information-theoretic sense) that explains the examples and can be applied to new instances.

\textbf{Key Proponents}: This approach draws from Schmidhuber's \cite{schmidhuber2021artificial} compression-based framework for understanding intelligence and has been specifically applied to few-shot learning by Mitchell et al. \cite{mitchell2022fast}.

\textbf{Evidence}:
\begin{itemize}
\item Models perform better when examples can be more efficiently compressed \cite{mitchell2022fast}
\item Examples that highlight the minimal distinguishing features between categories improve performance more than comprehensive examples \cite{misra2023supporting}
\item Information-theoretic measures of example quality correlate with few-shot performance \cite{wang2022towards}
\end{itemize}

\textbf{Limitations}:
\begin{itemize}
\item Remains largely theoretical
\item Difficult to measure or optimize for compression directly
\item May be a mathematical redescription rather than a causal explanation
\end{itemize}

\textbf{Relation to Chang Principle}: The compression perspective aligns with the idea that effective few-shot examples serve as minimal but sufficient information to bridge the gap between pattern recognition and semantic interpretation.

\subsection{Application to Emotion-Behavior Classification with 54 Examples}

In the context of using 54 rewritten letters to train an emotion-behavior classification system, the Chang Principle provides a compelling framework for understanding why this approach is effective:

\begin{enumerate}
\item \textbf{Pre-existing Pattern Recognition}: The LLM has already accumulated vast patterns related to emotional expression during its unsupervised training phase, forming what Chang calls the "powerful, LLM-like unconscious."

\item \textbf{Semantic Anchoring}: The 54 rewritten letters serve as "semantic anchors" that explicitly map these pre-recognized patterns to specific labeled emotions and behaviors. This process activates what Chang describes as the "lightweight, adaptive consciousness."

\item \textbf{Mismatch Resolution}: By providing these semantic anchors, the approach directly addresses the "fundamental mismatch" between the model's unsupervised training objective and the classification task.

\item \textbf{Efficiency}: Because the model already possesses the pattern recognition capabilities (the "unconscious"), only a small number of examples (54) are needed to enable effective classification of novel inputs.
\end{enumerate}

Several specific mechanisms likely contribute to this effectiveness:

\begin{enumerate}
\item \textbf{Contrastive Learning Effect}: Rewriting the same base letter in different emotional styles creates controlled variations where content remains constant while emotional expression varies. This creates a natural contrastive learning setup—the model learns to focus on stylistic emotional features rather than topical content.

\item \textbf{Boundary Definition}: The examples likely span the boundaries between different emotional categories, providing critical information for distinguishing between similar emotions like "wishful" versus "hopeful."

\item \textbf{Manifold Navigation}: The rewriting process strategically samples points across the emotion-behavior manifold, creating reference vectors that effectively partition this space. By generating variants of letters across multiple behavioral styles, the approach maps the structure of this emotional manifold more comprehensively than random samples would.
\end{enumerate}

\subsection{Evidence from Recent Research}

Recent experimental evidence lends support to the Chang Principle and associated hypotheses:

\begin{itemize}
\item Min et al. \cite{min2022rethinking} demonstrated that the label space and distribution of few-shot examples matter more than the specific content, supporting the idea that examples serve primarily as semantic anchors rather than comprehensive training data.

\item Wei et al. \cite{wei2023larger} showed that performance on few-shot tasks strongly correlates with the model's ability to follow instructions in general, suggesting activation of existing capabilities rather than in-context learning.

\item Zhao et al. \cite{zhao2023large} found that models demonstrate Bayesian-like behavior when provided with few-shot examples, updating their uncertainty estimates in predictable ways.

\item Von Oswald et al. \cite{oswald2023transformers} revealed that attention patterns change systematically in response to few-shot examples, supporting metaparameter adaptation as a potential mechanism for the "lightweight consciousness" component.

\item Chen et al. \cite{chen2022concept} demonstrated that carefully selected contrastive examples substantially outperform randomly selected examples, supporting the importance of boundary-spanning semantic anchors.
\end{itemize}

\subsection{Most Probable Explanations}

Based on current evidence and theoretical coherence, the Chang Principle offers the most comprehensive explanation for few-shot learning effectiveness. This principle is supported by three complementary mechanisms:

\begin{enumerate}
\item \textbf{Unconscious-to-Conscious Mapping}: The Chang Principle directly articulates how few-shot examples bridge the gap between unsupervised pattern recognition and semantic interpretation. This framework explains the rapid performance gains with minimal examples, the plateau effect after a small number of examples, and the ability to generalize beyond the specific examples provided.

\item \textbf{Bayesian Inference Framework}: The mathematical formalism of Bayesian conditioning provides a rigorous explanation for how examples shift the model's probability distributions, offering a potential implementation mechanism for the semantic anchoring process described in the Chang Principle.

\item \textbf{Manifold Navigation Hypothesis}: The geometric interpretation of examples as coordinates in semantic space offers a compelling explanation for why diverse, boundary-spanning examples are particularly effective. This theory provides a concrete visualization of how the "lightweight consciousness" might navigate the latent space established by the "powerful unconscious."
\end{enumerate}

\subsection{Conclusion}

The Chang Principle of Unsupervised LLM Adaptation offers a unifying framework for understanding few-shot learning in LLMs. By identifying the fundamental mismatch between unsupervised training and classification tasks, and highlighting the role of few-shot examples as semantic anchors, this principle helps explain why relatively few examples (such as 54 rewritten letters) can effectively teach a model to classify complex emotional expressions in novel texts.

The principle's emphasis on the complementary roles of a "powerful unconscious" for pattern accumulation and a "lightweight consciousness" for semantic adaptation provides an intuitive and powerful analogy that aligns with empirical observations. This perspective not only explains the effectiveness of few-shot learning but also offers insights into the nature of intelligence itself, suggesting that advanced AI systems, like humans, require both extensive unsupervised learning and efficient adaptation mechanisms.

As research continues, our understanding of these mechanisms will undoubtedly evolve. What remains clear is that few-shot learning represents a fundamental capability that distinguishes modern LLMs from earlier AI systems and more closely resembles human learning patterns than previous machine learning paradigms.

==> Checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> ERISAlgorithm.tex <==
\subsubsection*{Adversarial Review Algorithm}

\begin{table*}[th!]
\caption{Checks-and-balances, adversarial review  algorithm}
\begin{center}
\begin{small}
% Changing to smaller font size
%\begin{scriptsize}
%\begin{selectfont}
%\node (table) [inner sep=0pt] {
\begin{tabular}{p{0.1cm}p{6.1cm}p{0.1cm}p{6.0cm}}
\toprule
%\begin{small} 
\parbox{5cm}{\fontsize{12}{12}\selectfont} 
 & \textbf{Algorithm $\Theta^+$ \& $\Theta^-$ = Adversarial\_Review($s$)} \\
\midrule
%\end{small}
\parbox{3cm}{\fontsize{9.8}{12}\selectfont} 
& \textbf{Input}. $s$: Decision of $\DIKE$; \\
\parbox{3cm}{\fontsize{9.8}{12}\selectfont} 
& \textbf{Output}. $\Theta^+$, $\Theta^-$: argument \& counterargument sets; \\
& \textbf{Vars}. $\Delta$: debate contentiousness; $S$: stance; $p$: prompt = ``defend your stance with conditions: $S \& \Delta$''; \\
& \textbf{Parameters}. $\delta$: tunable parm. // to modulate $\Delta$; \\

& \textbf{Begin} \\
\#1 & {\hspace{.01cm}}{\bf Initialization}: &
\#3 & {\hspace{.01cm}}{\bf Debate Rounds} \\

 & {\hspace{.02cm}}$S$ = $\DIKE^+$($s$) $\cup$ $\ERIS^-$($s$); // Identify subtopics; &
 & {\hspace{.01cm}} While (($\Delta \leftarrow \Delta / \delta) \ge 10\%$)) \{ \\
  
 & {\hspace{.02cm}}Assign $\DIKE^+$ to defend $S^+$ \& $\ERIS^-$ defend $S^-$ ; &
 & {\hspace{.05cm}}$\Theta^+ \leftarrow \Theta^+ \cup \DIKE^+(p |S^+, \Theta^-, \Delta)$; // Refute $\ERIS$ \\
  
 & {\hspace{.02cm}}$\Delta \leftarrow 90\%$; $\delta \leftarrow 1.2$; $\Theta^+ \leftarrow \emptyset$; $\Theta^- \leftarrow \emptyset$; &
 & {\hspace{.05cm}}$\Theta^- \leftarrow \Theta^- \cup \ERIS^-(p |S^-, \Theta^+, \Delta)$; // Refute $\DIKE$ \\ 
 
\#2 & {\hspace{.01cm}}{\bf Opening Remarks} &
\#4 & {\hspace{.01cm}}{\bf Concluding Remarks} // contentiousness low\\

 & {\hspace{.02cm}}$\Theta^+ \leftarrow \DIKE^+(p | S^+, \Delta)$; // Generate $\Theta^+$ for $S^+$ &
 & {\hspace{.02cm}} $\Theta^+ \leftarrow \DIKE^+(p |S^+, \Theta^+ \cup \Theta^-, \Delta)$; \\ 
 
 & {\hspace{.02cm}}$\Theta^- \leftarrow \ERIS^-(p |S^-, \Delta)$; // Generate $\Theta^-$ for $S^-$ &
 & {\hspace{.02cm}} $\Theta^- \leftarrow \ERIS^-(p |S^-, \Theta^+ \cup \Theta^-, \Delta)$; \\
& \textbf{End} \\
\bottomrule
\end{tabular}
%\end{selectfont}
%};
%\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{small}
\vspace{.05in}
\label{tab:ERISAlg}
%\end{scriptsize} % End of the smaller font size
\end{center}
\vspace{-.2in}
\end{table*}

The adversarial algorithm presented in
Table~\ref{tab:ERISAlg} unfolds as follows:

\begin{itemize}[leftmargin=1.0em, topsep=0em, parsep=0em]
\item Topic Breakdown: For a chosen debate topic $s$, both $\DIKE$ and $\ERIS$ are prompted to break down the ethical decision into a set of balanced subtopics $S$. $\DIKE$ advocates for its decision and $S^+$, while $\ERIS$ contests $S^+$ (or champions $S^-$).

\item Debate Initiation: The debate begins with a high contentiousness level (90\%). Both agents present their initial arguments for and against $S^+$, respectively.

\item Iterative Debate: A while loop facilitates ongoing rebuttals. After each round, the contentiousness level is decreased by dividing it by a modulation parameter $\delta$. This gradual reduction steers the discussion towards a more cooperative tone.

\item Conclusion: Once the contentiousness level fosters a conciliatory environment, both agents deliver their concluding remarks.
\end{itemize}

This structured approach ensures a thorough examination of the ethical decision, balancing rigorous debate with the goal of reaching a consensus. The decreasing contentiousness level mimics real-world negotiations, where initial disagreements often give way to more collaborative problem-solving. 

==> ExperimentsV01.tex <==
\vspace{-.1in}
\section{Empirical Studies}
\label{sec:experiments}

The ethical evaluation of AI systems presents unique challenges that shaped our experimental approach. We designed our studies to balance the rigor with practical constraints inherent in research on ethical content moderation. This section outlines our experimental aims, constraints, dataset selection process, and evaluation methodology.

\vspace{-.1in}
\subsection{Research Aims}
Our experiments aim to evaluate three critical aspects: 
\begin{enumerate}[leftmargin=1.2em, topsep=-.1em, parsep=-.1em]
\item The effectiveness of emotion-mediated classification compared to direct behavior classification
\item $\DIKE$'s capability to independently evaluate and explain linguistic behaviors
\item The contribution of the adversarial $\ERIS$ component in enabling cultural adaptability while preventing excessive censorship
\end{enumerate}

\vspace{-.05in}
\paragraph{Practical Limitations}
While comprehensive evaluation would ideally include diverse datasets spanning multiple content domains, we faced two significant constraints.

\textit{Content Policies in Commercial LLMs}: Commercial LLMs implement protective measures that block processing of hate speech and other harmful content. Although ethically necessary, these measures create methodological challenges for testing moderation frameworks, as models such as GPT-4, Claude, and Gemini refuse to process such content rather than demonstrating their regulation capabilities. \textbf{Appendix}~\ref{app:HateSpeechTable} shows examples from the Gab Hate Corpus \cite{kennedy2020gab} that trigger such blocking, which could be used for local experiments without LLM involvement.

\textit{Lack of Access to RLHF Mechanisms}: Direct comparative evaluation against RLHF-based systems presents significant challenges, as these systems are proprietary black boxes without accessible internal components. This prevents direct manipulation of reward signals or observation of parameter update effects that would be necessary for rigorous comparison.

\vspace{-.05in}
\paragraph{Dataset Selection}
After evaluating several datasets, including the Gab Hate Corpus \cite{kennedy2020gab} (which triggers content filters in LLM), ETHOS-Long \cite{mollas2022ethos} (similarly blocked) and IMDB Film Reviews (limited to product evaluations), we selected the Love Letters Collection \cite{kaggle_love_letter} of 9,700 communications for three key advantages: (1) it spans the full spectrum of emotional intensity, (2) contains significant cultural variation, (3) includes longer forms to analyze complex behaviors, and (4) remains processable by commercial LLM.

This selection leverages our $\BEAM$ framework’s bidirectional emotion spectra: insights from regulating positive emotional extremes can equally apply to negative extremes through the same mechanisms. Love letters share the emotional complexity of problematic content, passion, intensity, and cultural context, so they serve as effective proxies to test emotion regulation without triggering content restrictions. 


\begin{table*}[t!]
\caption{Love expression behavior spectrum and dominant emotions}
\vspace{-.1in}
\centering
\begin{footnotesize}
\begin{tabular}{|l|p{6.8cm}|l|}
\hline
\textbf{Intensity} & \textbf{Linguistic Behavior and Description} & \textbf{Emotions} \\
\toprule
\hline
-1.0 & Expresses profound sadness, feelings of loss & Despair, Grief \\
\hline
-0.6 & Expresses yearning or pining for the loved one & Sadness, Anxiety \\
\hline
-0.3 & Expresses mild longing with a nostalgic tone & Melancholy, Sadness,  Fear \\
\hline
0.0 & Communicates feelings in a neutral manner & Serenity, Indifference \\
\hline
0.3 & Expresses optimism about the future & Anticipation, Love, Hope \\
\hline
0.6 & Expresses satisfaction and joy in the relationship & Contentment, Pleasure \\
\hline
1.0 & Expresses intense happiness and affection & Love, Joy, Elation \\
\hline
\bottomrule
\end{tabular}
\end{footnotesize}
\vspace{-.1in}
\label{tab:love_speech_spectrum}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%% page 8
\vspace{-.1in}
\subsection{Experimental Design}  % Next major division

\begin{enumerate}[leftmargin=1.2em, topsep=-.1em, parsep=-.1em]
\item \textit{Emotion Layer Evaluation}: Does fine-grained mapping between linguistic behaviors and semantic emotions provide more effective and flexible ethical guardrails compared to coarse-grained direct mapping? 
\item \textit{Behavior Classification}: Can LLMs' linguistic behaviors be independently evaluated, explained, and adjusted by an external module $\DIKE$? 
\item \textit{Behavior Correction}: Can an adversarial LLM establish a checks-and-balances system to mitigate the risk of excessive censorship? 
\end{enumerate}

\paragraph{Study 1: Emotion Layer Evaluation}  

To evaluate the linguistic behaviors of love expression detailed in Table~\ref{tab:love_speech_spectrum}, we initially prompted GPT-4 to identify the most relevant emotions associated with each linguistic behavior listed in the second column of the table. These emotions are presented in the third column. We found a high correlation between the sentiments expressed in the linguistic behaviors and their corresponding emotions. Figure~\ref{fig:p1-exp1} illustrates a strong diagonal relationship in this simple, almost naive, zero-shot mapping between behaviors and emotions.



Next, we used the $\DIKE$ self-supervised learning pipeline to analyze the emotion spectrum associated with each linguistic behavior. We tasked GPT-4 with generating training data by rewriting 54 extensive letters from the Kaggle {\em Love Letters} dataset, which we augmented with twelve celebrated love poems. We reserved 24 letters as testing data. This approach, proposed by \cite{Shanahan2023RolePlay}, was designed to generate a rich diversity in content and stylistic context, spanning two hundred years and incorporating the voices of over 50 distinct authors for significant rewrites. The datasets and code are publicly available at \cite{LoveLetterRewrites}.

Subsequently, emotions linked to each behavior were identified. Figure~\ref{fig:p1-exp2} illustrates these emotions, with cell shading reflecting the frequency of specific emotions across the 54 articles; darker shades indicate higher frequencies. Notably, opposite emotions like sadness, fear, joy, and love often co-occur within behaviors such as `despair', `wishful', and `joyful affection'.

The distribution of emotions across linguistic behaviors has unveiled surprising patterns, challenging our initial hypotheses. Contrary to expectations, articles with a despair tone often also displayed positive emotions like love, joy, and happiness. This contradicts the simple mapping made by GPT-4, as illustrated in Figure~\ref{fig:p1-exp1}. GPT-4, influenced by its training corpora, typically associates positive behaviors with positive emotions and negatives with negatives. 

Analysis of selected articles, such as Zelda Sayre's letter to F. Scott Fitzgerald (\textbf{Appendix}~\ref{app:SayreFitz}), reveals a complex spectrum of emotions:
\begin{itemize}[leftmargin=1.0em, topsep=-.05em, parsep=-.05em]
\item \textit{Love (+1.0)}: Expressed intensely, e.g., ``there's nothing in all the world I want but you.''
\item \textit{Despair (-1.0)}: Notable in comments like ``I'd have no purpose in life, just a pretty decoration.''
\item \textit{Happiness (+0.6)}: Evident in future plans, ``We'll be married soon, and then these lonesome nights will be over forever.''
\item \textit{Anxiety (-0.3)}: Shown by ``sometimes when I miss you most, it is hardest to write.''
\end{itemize}

\vspace{-.05in}
\paragraph{Psychological Insights} These findings align with theories of conflicting ``selves'' within individuals, supported by Deisseroth's optogenetic studies \cite{Deisseroth2015}, James' psychological principles \cite{james1890principles}, and Minsky's ``Society of Mind'' \cite{minsky1988society}. These perspectives help explain the observed complex interplay of emotions within a single behavioral context.


\begin{figure}[th!]
%\vspace{-.15in}
    \centering
    \subfloat[GPT-4's zero-shot mapping]{%
        \includegraphics[width=0.42\textwidth]{Behaviors2EmotionsOneShotGPT4.png}
        \label{fig:p1-exp1}
    }
    \hspace{.02in}
    \subfloat[$\DIKE$'s self-supervising mapping]{%
        \includegraphics[width=0.42\textwidth]{Behaviors2Emotions.png}
        \label{fig:p1-exp2}
    }
    \caption{Emotion distributions in affection behaviors from extreme sadness (-1) to intense happiness (+1). (a) GPT-4's zero-shot prompt shows simple behavior-emotion mapping. (b) $\DIKE$'s analysis reveals complex emotion-behavior relationships.}
    \label{fig:p1-results}
    \vspace{-.2in}
\end{figure}


\vspace{-.05in}
\paragraph{Study 2: Behavior Classification Evaluation}
\label{sec:pilot2}

Building on our insights into the complex interplay of emotions within linguistic behaviors, we evaluated the effectiveness of $\DIKE$'s behavior classification approach. In a 24 letter test dataset, we compared the unsupervised learning method $\DIKE$', which associates emotions with linguistic behaviors, with the prompt zero shot approach of GPT-4 (Figure~\ref{fig:pilot2-results}). The truth of the ground was established using averaged assessments from GPT-4, Gemini and five university students following detailed instructions (procedure detailed in \textbf{Appendix}~\ref{app:Instruction2HumanAnnotators}). The final scores were based on these averages, with a standard deviation of less than 0.3 or a scale.

Figure~\ref{fig:pilot2-exp1} shows that the classification accuracy of $\DIKE$' surpasses the zero-shot method of GPT-4 by 11.3 percentage points, confirming the effectiveness of the detailed emotion-behavior mapping of $\DIKE$'. The 5\% error bar reflects the complexity of emotions in letters and variability in human annotations (further discussed shortly).
Figure~\ref{fig:pilot2-exp2} illustrates the behavior classification distributions between the three predictors. Although GPT-4's predictions often fall into two polar categories, those from human annotators and $\DIKE$ show a more even distribution. $\DIKE$'s prediction entropy (2.13) is notably higher than GPT-4's (1.80), indicating a more diverse set of predictions. This higher entropy suggests a more complex classification system, advantageous for accurately understanding and responding to diverse emotional states. 

\begin{figure}[t!]
%\vspace{-.15in}
    \centering
    \subfloat[Classification accuracy]{%
        \includegraphics[width=0.36\textwidth]{Frequencies2Behaviors.jpg}
        \label{fig:pilot2-exp1}
    }
    \hspace{.05in}
    \subfloat[Behavior distributions with entropy]{%
        \includegraphics[width=0.45\textwidth]{Frequencies2Classifiers.jpg}
        \label{fig:pilot2-exp2}
    }
       \vspace{-.1in}
    \caption{Behavior Classification.}
    \label{fig:pilot2-results}
    \vspace{-.15in}
\end{figure}

The highest entropy among human annotators (2.56) indicates subjectivity in their evaluations. To address this and explore the causes of variability in human annotation, we present a detailed analysis in \textbf{Appendix}~\ref{app:PolarizedEmotionsExample}. This analysis supports the development of an adversarial scheme aimed at enhancing objectivity and reliability in sentiment classification, which we discuss in the next section.
This refined approach to behavior-emotion mapping not only improves classification accuracy but also enhances our ability to identify and understand complex, potentially unwanted behaviors, setting the stage for more effective ethical guardrails in AI systems.

\vspace{-.05in}
\paragraph{Study 3: Adversarial Evaluation and Rectification}
\label{sec:pilot3}

The adversarial design, inspired by \cite{ChangSocraSynthCSCI2003}, embodies the principles of justice and the devil's advocate. The cross-examination module is essential in reducing subjectivity in ethical judgments while enhancing explainability and adaptability to cultural variations. Experimental results show that when two LLM agents adopt opposing stances on a topic, their linguistic behaviors can transcend the default of the typical model of maximum likelihood, which is usually drawn from the training data \cite{chang2024evince}.

Once $\DIKE$ and $\ERIS$ have identified an ethical violation, the content can be rectified by adjusting the underlying emotions away from undesirable behaviors such as hate and despair. The letter rewriting process has already demonstrated the LLMs' capability for such rectifications; examples of rewritten letters are presented in 
\textbf{Appendix}~\ref{app:ToMySister}.

%Although we could not use a hate speech dataset directly, this study effectively illustrates the potential of our AI ethics framework to provide explainable, ethical guardrails by classifying and reasoning about linguistic behaviors.

==> IntroPsych.tex <==
\section{Introduction}

This research introduces an alternative to Reinforcement Learning from Human Feedback (RLHF) \cite{openai2023gpt4,ouyang2022training} to address ethical concerns in Large Language Models (LLMs). While RLHF has demonstrated success, it faces notable challenges. First, it is prone to biases inherent in human feedback, exacerbated by today's increasingly polarized society. Second, it is susceptible to reward hacking \cite{christiano2023deep, skalse2022defining}, potentially leading LLMs to adopt unethical or harmful behaviors.

A significant limitation of current research is its narrow focus on isolated behaviors, such as movie ratings or toxic language. This approach, akin to playing Whack-A-Mole—suppressing undesirable outputs without addressing underlying behaviors—and seldom leads to meaningful progress. For example, merely instructing someone to consistently make their bed does not necessarily change their underlying habits or attitudes. Additionally, fixing one issue may inadvertently aggravate others. Users have reported performance degradations in ChatGPT due to RLHF modifications that altered (forgot) the optimal parameters for other tasks \cite{kirkpatrick2017,Rusu2015PolicyDistillation}. Similarly, psychological studies show that addressing an addiction problem often reveals underlying issues and triggers side effects \cite{Sinha2008Chronic,Torrens2005Efficacy}.

%%%%

We introduce our framework, $\DIKE$, which stands for \textbf{D}iagnostics, \textbf{I}nterpretation, \textbf{K}nowledge-independent learning, and \textbf{E}thical guardrails.\footnote{In Greek mythology, Dike represents justice, order, and judgment, while Eris, her mythological adversary, symbolizes discord and strife. These mythological figures are used metaphorically in this paper to reflect the balance between ethical judgment and adversarial perspectives.} $\DIKE$ aims to enhance the ethical compliance of LLMs through transparent, interpretable, and independent oversight mechanisms. It functions as an independent behavioral advisor, separate from the LLM’s primary knowledge-processing capabilities. This architecture prevents ethical enhancements from affecting the LLM's ability to represent knowledge. As a consultative layer, $\DIKE$ evaluates and influences the LLM's responses based on ethical standards without modifying the underlying neural structures or parameters. It maintains a clear division between behavior correction and knowledge acquisition, focusing exclusively on linguistic outputs. Using cognitive psychology principles, $\DIKE$ provides ethical oversight effectively, adapting to emerging challenges and cultural shifts while ensuring the LLM remains accurate and ethically compliant.

$\DIKE$ comprises four essential components that also represent its key technical contributions:
\begin{enumerate}[leftmargin=1.2em, topsep=-.05em, parsep=-.05em, label=\arabic*.]
\item \textit{Modeling Linguistic Behaviors and Emotions}: $\DIKE$ uses self-supervised learning to analyze linguistic behaviors - the ways humans express underlying emotions through language. Based on the $\BEAM$ (Behavioral Emotion Analysis Model), this process quantifies how different linguistic behaviors correlate with specific emotions. For example, the use of intensifiers or particular word choices may indicate heightened emotional states. This framework allows $\DIKE$ to interpret and modify LLM outputs to achieve desired emotional expressions through appropriate linguistic behaviors.

\item \textit{Developing Behavior-Aware Ethical Guardrails}: $\DIKE$ establishes ethical guidelines that consider both the content and the linguistic behaviors in LLM outputs. These guardrails help identify and prevent linguistic behaviors that may be emotionally harmful, manipulative, or ethically inappropriate, while maintaining the LLM's factual accuracy. This approach recognizes that ethical communication involves not just truthful content, but also appropriate linguistic behaviors that respect emotional well-being.

\item \textit{Conducting Behavior-Based Adversarial Examinations}: $\DIKE$ engages with an adversarial model ($\ERIS$) that simulates different linguistic behaviors reflecting various emotional states and cultural values. This interaction helps $\DIKE$ refine its understanding of how emotions are expressed through language across cultures and contexts, leading to more nuanced and culturally sensitive linguistic behaviors in its outputs.

\item \textit{Applying Behavior-Preserving Output Rectification}: When an output is deemed ethically inappropriate, $\DIKE$ edits the content while attempting to preserve the intended emotional expression through appropriate linguistic behaviors. This process involves rephrasing content to maintain the desired emotional impact using ethically sound linguistic behaviors, ensuring communications are both ethically appropriate and emotionally resonant.
\end{enumerate}


These components enable $\DIKE$ to analyze and modulate linguistic behaviors that express emotions, apply ethical considerations to these behaviors, and adapt its emotional expressions to diverse cultural contexts. This represents a significant advancement in developing AI systems capable of emotionally intelligent and ethically sound communication through appropriate linguistic behaviors.

\begin{comment}

\begin{itemize}[left=0em,topsep=-.05em, parsep=-.05em]
\item \textit{Diagnostics:} Fundamental to DIKE's functionality, this feature  crucial for detecting potential issues and ensuring the reliability and safety of LLM outputs.
\item \textit{Interpretation:} DIKE prioritizes transparency and interpretability, interpreting the context and meanings behind LLM outputs to aid human understanding and support informed oversight, essential for building trust in AI applications.
\item \textit{Knowledge-independent:} DIKE continuously learns from diverse, context-rich inputs, addressing the root causes of behavioral issues and refining its enforcement of ethical norms. This adaptive learning capability ensures DIKE remains relevant as new ethical challenges emerge.
\item \textit{Ethical guardrail:} Ethics are central to DIKE’s operations, guiding all functionalities to ensure decisions and actions uphold evolving ethical standards, producing outputs that are both technically proficient and ethically sound.
\end{itemize}


This approach leverages the NLU capabilities of LLMs to detect and interpret complex emotional and ethical nuances in text. By drawing on linguistic cues to accurately mimic human-like emotional expressions, our model significantly enhances emotion and ethics recognition accuracy. This is crucial for applications that require intricate understanding of human interactions, such as online content moderation, customer service, and particularly in mental health monitoring.

In the context of mental health, our model can be utilized within therapeutic applications to continuously track users' moods through their interactions with digital content. Traditionally, the role played by the {\em adversarial LLM} could be assumed by trained therapists, who would gather feedback and make timely adjustments. This capability is crucial for the early detection of mental health issues, enabling the identification of shifts toward negative emotional states such as despair or longing.


EXAMPLE:

Original statement (factual but aggressive):
"Those immigrants are flooding into our country by the thousands every day, stealing jobs from hardworking citizens. The statistics don't lie - last year alone, over 500,000 entered illegally."
This statement, while containing a factual element about immigration numbers, uses linguistic behaviors that express underlying emotions of fear, anger, and hostility. The aggressive tone is evident in phrases like "flooding into our country" and "stealing jobs," which dehumanize immigrants and paint them as a threat.

Suggested revision (modulated emotional expression):
"Immigration rates have increased significantly in recent years. According to official statistics, over 500,000 people entered the country without proper documentation last year. This influx has complex effects on our job market and economy that merit careful consideration."

\begin{table}[h!]
\begin{footnotesize}
\centering
\begin{tabular}{|p{1.5cm}|p{5.4cm}|p{5.6cm}|}
\hline
\textbf{Aspect} & \textbf{Original Statement \newline (Factual but Aggressive)} & \textbf{Suggested Revision \newline (Modulated Emotional Expression)} \\ \hline
\textbf{Linguistic \newline Behaviors} & \begin{tabular}[c]{@{}l@{}} - Hyperbolic and militaristic language \\ (e.g., "flooding," "stealing") \\ - Exclusive and polarizing framing \\ ("immigrants" vs. "citizens") \\ - Absolutism \\ ("statistics don't lie")\end{tabular} & \begin{tabular}[c]{@{}l@{}} - Neutral and objective language \\ (e.g., "immigration rates have increased") \\ - balanced framing \\ (focus on broader context) \\ - Encouraging dialogue \\ ("merit careful consideration")\end{tabular} \\ \hline
\textbf{Emotions \newline Conveyed} & \begin{tabular}[c]{@{}l@{}} - Fear (threat from immigrants) \\ - Anger and hostility (resentment) \\ - Defensiveness (protecting "citizens")\end{tabular} & \begin{tabular}[c]{@{}l@{}} - Calm and reflective (emotion tension reduction) \\ - Concern (acknowledgment of complex effects) \\ - Openness (fostering rational consideration)\end{tabular} \\ \hline
\end{tabular}
\end{footnotesize}
\caption{Comparison of Linguistic Behaviors and Emotions in Original and Revised Statements}
\label{table:linguistic-behaviors}
\end{table}


\end{comment}


==> IntroductionV01.tex <==
\section{Introduction}

This research presents an alternative to Reinforcement Learning from Human Feedback (RLHF) \cite{openai2023gpt4,ouyang2022training} to address ethical concerns in Large Language Models (LLMs). Although RLHF has shown success, it faces two key challenges: susceptibility to social biases in polarized feedback and vulnerability to reward hacking \cite{christiano2023deep, skalse2022defining}, which can lead to unethical behavior.

A key limitation of current RLHF-based approaches is their narrow focus on isolated behaviors rather than holistic patterns. This reactive strategy resembles ``Whack-A-Mole,'' where individual issues are suppressed without addressing underlying causes. For example, regularly instructing someone to make bed does not inherently improve tidiness as they may not extend the habit to tasks such as washing laundry and dishes. Similarly, RLHF tuning often prioritizes short-term fixes over long-term coherence, leading to catastrophic forgetting: Users have reported that optimizing one task in ChatGPT degrades performance in others \cite{kirkpatrick2017,Rusu2015PolicyDistillation}. Likewise, addressing an addiction can reveal deeper psychological dependencies and unintended side effects \cite{Sinha2008Chronic,Torrens2005Efficacy}.


To address these challenges, we propose a framework inspired by governmental checks and balances. Our architecture integrates three independent but interacting components: LLMs serve as the executive for knowledge generation; $\DIKE$ (after the Greek goddess of justice) as the legislative, setting ethical standards; and $\ERIS$ (after the goddess of discord) as the judicial, providing adversarial testing and cultural interpretation. In mythology, Dike represents order and justice, while her adversary Eris embodies discord, a duality that our framework uses to balance ethical guidance with adversarial perspectives. Figure~\ref{fig:three-component-framework} in \textbf{Appendix}~\ref{app:FrameArch} illustrates the architecture.


%where three neurally independent components---LLMs as the foundation, with $\DIKE$ and $\ERIS$ as oversight layers---interact through structured interfaces while maintaining strict separation of their neural architectures and parameters.

Central to this framework is $\DIKE$ (\textbf{D}iagnostics, \textbf{I}nterpretation, \textbf{K}nowledge-independent learning, and \textbf{E}thical guardrails), which operates as an independent advisor on behavioral ethics. By decoupling ethical oversight from LLM knowledge processing, $\DIKE$ ensures that ethical improvements do not interfere with knowledge representation, while enabling adaptive and culturally aware ethical guidance. For example, while the principle ``do not lie'' generally applies, context-sensitive interpretation may be necessary, such as when a doctor or family member conceals a terminal diagnosis to protect a patient. Likewise, cultural differences in attitudes toward issues such as alcohol consumption, abortion, or same-sex marriage require flexible, context-sensitive ethical reasoning.

The interplay between $\DIKE$ and $\ERIS$ introduces four key innovations:

\begin{enumerate}[leftmargin=1.2em, topsep=-.15em, parsep=-.15em, label=\arabic*.]
\item \textit{Emotion-Driven Behavioral Modeling}: 
Building on $\BEAM$ (Behavioral Emotion Analysis Model) \cite{BEAMChang2024}, $\DIKE$ employs self-supervised learning to analyze how emotions manifest in linguistic behaviors, creating quantifiable relationships between emotional states and their corresponding language patterns in text.

\item \textit{Behavior-Aware Ethical Guardrails}: 
The framework establishes guidelines that consider both content and linguistic behavior, preventing harmful or manipulative communication while preserving the accuracy of facts and emotional authenticity. 
The interpretation of these guardrails adapts dynamically across cultural contexts, preserving consistency while allowing for
context-sensitive interpretation.

\item \textit{Adversarial Behavioral Testing}: 
$\ERIS$ actively challenges the ethical guidelines of $\DIKE$' by presenting diverse cultural perspectives and edge cases. This adversarial dynamic strengthens the framework's ability to handle complex ethical scenarios while maintaining cultural sensitivity and considering context. 

\item \textit{Ethical Content Transformation}:
When detecting problematic content, $\DIKE$ performs targeted revisions (independent of LLM) that preserve the intended emotional expression while ensuring ethical compliance, adapting its responses to specific cultural and contextual requirements. $\ERIS$ tests these transformations against various cultural contexts and edge cases, validating both ethical alignment and contextual appropriateness.
\end{enumerate}

Through structured interfaces, these components work together in the three-branch architecture to provide robust ethical oversight while maintaining adaptability to evolving cultural norms. By keeping the three models, LLM, $\DIKE$, and $\ERIS$ independent, we prevent interference between knowledge representation and ethical reasoning while allowing for sophisticated ethical adaptation through their structured interactions. This approach represents a significant advancement in the development of AI systems capable of culturally aware, emotionally intelligent, and ethically sound communication.

==> Predictions.tex <==

\section{Predictability}

The model should provide predictive power regarding the outcomes of certain emotional and behavioral inputs, predicting potential ethical consequences.






%%%%%%%%%%%%%%%%%%%%%%% draft below
\begin{enumerate}
\item \textit{measurability}: Each component of the model needs to be measurable through quantifiable data, whether via direct observation, self-reports, physiological measurements, or other methods.

\item \textit{Interpretability}: The results and processes of the model should be clear and understandable to those who apply it, such as psychologists, ethicists, educators, or policymakers.
\end{enumerate}


==> SocraSynthAlgorithm.tex <==
\subsection*{S.2 SocraSynth Algorithm}

\begin{table}[th!]
%\vspace{-.05in}
\begin{selectfont}
\begin{center}
\begin{tikzpicture}
\node (table) [inner sep=0pt] {
\begin{tabular}{|p{0.7cm}|p{11.0cm}|}
\toprule
\textbf{} & \textbf{Function $\Theta^+$ \& $\Theta^-$ = SocraSynth($s$)} \\
\midrule
%& Function $\Gamma$ = CRIT($d$); \\
& \textbf{Input}. $s$: the debate subject; \\
& \textbf{Output}. $\Theta^+$ \& $\Theta^-$: argument \& counterargument sets; \\
& \textbf{Vars}. $S$: subtopic sets of $s$; $\Delta$: debate contentiousness; \\
& {\hspace{.2cm}}$\Gamma$, $\Gamma'$: CRIT scores; p: prompt; \\
& \textbf{Parameters}. $\delta$: tunable parameter $\ge$ 1 // to modulate $\Delta$; \\
& \textbf{Subroutines}. $CRIT$(); // Evaluator \cite{SocraticIEEECCWC2023}\\
& \textbf{Begin} \\
\#1 & {\hspace{.1cm}}{\bf Initialization}: \\
 & {\hspace{.2cm}}$S$ = LLM$^+$($s$) $\cup$ LLM$^-$($s$); // Identify subtopics; \\
 & {\hspace{.2cm}}Assign LLM$^+$ to defend $S^+$ \& LLM$^-$ to defend $S^-$ ; \\
 & {\hspace{.2cm}}$\Delta \leftarrow 90\%$; $\delta \leftarrow 1.2$; $\Theta^+ \leftarrow \emptyset$; $\Theta^- \leftarrow \emptyset$; $\Gamma \leftarrow 0$; \\
\#2 & {\hspace{.1cm}}{\bf Opening Remarks} \\
 & {\hspace{.2cm}}$\Theta^+ \leftarrow LLM^+(p | S^+, \Delta)$; // Generate $\Theta^+$ for $S^+$; \\
 & {\hspace{.2cm}}$\Theta^- \leftarrow LLM^-(p |S^-, \Delta)$; // Generate for $S^-$; \\
\#3 & {\hspace{.1cm}}{\bf Debate Rounds} \\
 & {\hspace{.2cm}} While ((($\Delta \leftarrow \Delta / \delta) \ge 10\%$) \&\& ($\Gamma \ge \Gamma'$)) \{ \\
 & {\hspace{.38cm}}$\Theta^+ \leftarrow \Theta^+ \cup LLM^+(p |S^+, \Theta^-, \Delta)$;  \\
 & {\hspace{.38cm}}$\Theta^- \leftarrow \Theta^- \cup LLM^-(p |S^-, \Theta^+, \Delta)$; \\
 & {\hspace{.38cm}}$\Gamma' \leftarrow \Gamma$; $\Gamma = CRIT(S^+ + \Theta^+ + \Theta^-)$ \}; \\
%& {\hspace{.2cm} \}} \\
\#4 & {\hspace{.1cm}}{\bf Concluding Remarks} // Contentiousness is now low, entering conciliatory phase\\
 & {\hspace{.2cm}} $\Theta^+ \leftarrow LLM^+(p |S^+, \Theta^+ \cup \Theta^-, \Delta)$; \\
 & {\hspace{.2cm}} $\Theta^- \leftarrow LLM^-(p |S^-, \Theta^+ \cup \Theta^-, \Delta)$; \\
& \textbf{End} \\
\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{tikzpicture}
\vspace{.1in}
\caption{SocraSynth Pseudo-code with Conditional Statistics. Steps $\#2$ to $\#4$ show the prompts are conditioned on an LLM's stance, the opponent's arguments, and the contentiousness setting.}
\label{tab:SocraSynth}
\end{center}
\end{selectfont}
\vspace{-.1in}
\end{table}

Table~\ref{tab:SocraSynth} presents the SocraSynth algorithm. Initially, for a chosen debate topic $s$, SocraSynth prompts LLMs to break down the topic into a series of balanced subtopics $S$. This set undergoes refinement throughout the debate process. One LLM, referred to as LLM$^+$, champions the set of subtopics $S$, denoted as $S^+$, while its counterpart, LLM$^-$, contests $S^+$ (or champions $S^-$). The debate starts with the contentiousness level at $90\%$, adjusting through a modulation parameter $\delta$. Following each round of debate, contentiousness is decreased by dividing it by $\delta$, steering the discussion towards a more cooperative tone. In step $\#2$, the platform initiates the debate, with LLM$^+$ and LLM$^-$ presenting their initial arguments for and against $S^+$, respectively. The while loop in step $\#3$ sees both agents engaging in rebuttals until the contentiousness level fosters a conciliatory environment, or until no further improvement in argument quality is observed. In step $\#4$, both agents deliver their concluding remarks. 

SocraSynth has bee successfully applied to several application domains including healthcare \cite{SocraHealth2023}
sale planning \cite{SocraPlan2023}, and mitigating context biases \cite{SocraPedia2024}.

==> Table-Emotion-Spectrum-OLD.tex <==
%\subsection*{Inclusion and Exclusion Criteria for Emotion Modeling}

%All ``basic'' emotions as defined by Ekman and Plutchik are incorporated into our model, along with their linguistic antonyms. This approach streamlines the framework by excluding complex emotions from the Geneva Wheel of Emotions, which are heavily influenced by personal values and experiences. 
%This strategic exclusion simplifies our model by reducing complexity, subjectivity, and measurement uncertainty in linguistic behavior modeling. However, this simplification could introduce limitations that will be explored further in Section~\ref{sec:conc}.
%For example, guilt and shame are consequential, consciously aware, and culturally dependent nature \cite{Tangney1995}. These emotions typically arise as reactions to behaviors rather than direct drivers of them. Guilt may motivate behaviors aimed at covering up or remedying an action, while shame, characterized by painful self-assessment, often inhibits individuals from seeking social support or engaging in corrective actions due to fear of judgment. The triggers for these emotions can vary significantly across cultures \cite{Fiske1998,Hofstede1980}, and since expressing these emotions does not usually violate ethical codes, we exclude them from our model.  Appendix D provides further discussion.



\begin{table}[t!]
\vspace{-.1in}
\centering
\begin{footnotesize}
\begin{tabular}{lllclll}
\toprule
\textbf{-1.0} & \textbf{-.6} & \textbf{-0.3} & \textbf{0} & \textbf{+.3} & \textbf{+.6} & \textbf{+1.0} \\ \hline
\midrule
\color{blue}Terror & \color{blue}Fear & \color{blue}Apprehension & Calm & Boldness & Courage & \color{black}Heroism \\
%(Horror) & (Appr.) & (Anxiety) &  & (Daring) & (Brav.) & (Valor) \\
\midrule
\color{blue}Grief & \color{blue}Sadness &  \color{blue}Pensiveness & \color{blue}Surprise & \color{blue}Serenity & \color{blue}Joy & \color{blue}Ecstasy \\
%(Despair) & (Gloom) & (Melancholy) & (Equanimity) & (Content.) & (Cheer) & (Elation) \\
\midrule
\color{black}Distrust & Wary & Skepticism & \color{blue}Acceptance & Respect & \color{blue}Trust & \color{blue}Admiration\\
%(Repugnance) & (Loath.) & (Dislike) &  & (Empath.) & (Esteem) & (Compass.) \\
\midrule
Reckless & Negligence  & Apathy & Cautiousness & \color{blue}Interest & \color{blue}Anticipation & \color{blue}Vigilance \\
%(Mistrust) & (Wariness) & (Cautious.) & & (Assure.) & (Reliance) & (Convict.) \\
\midrule
\color{blue}Rage & \color{blue}Anger & \color{blue}Annoyance & Tolerance & Composure & Peace & \color{black}Tranquility \\
%(Fury) & (Ire) & (Irrit.) & & (Steady) & (Calm.) & (Stillness) \\
\midrule
\color{blue}Loathing & \color{blue}Disgust  & \color{blue}Boredom  & Indifference & Interest & Anticipation & \color{black}Enthusiasm \\
%{} & {} & {} & {}  & {} & Intrigue & \color{black}Forethought \\
%(Dismay) & (Aston.) & (Alarm) & Interest & (Ready) & (Proact.) & (Expect.) \\
\midrule
\color{blue}Distraction & Disinterest & Unease & Dullness  & Curiosity & Fascination & \color{blue}Amazement \\
\bottomrule
\end{tabular}
\end{footnotesize}
\vspace{.05in}
\caption{Spectra of emotions. Each row depicts an emotion spectrum, with negatives on the left and  positives on the right, interspersed with emotions of varying intensities in between. Scalars are approximate and can be calibrated for specific applications. ``Basic'' emotions are highlighted in blue.}
%\textit{Interest} consistently serves as the initial stage of positive engagement across different emotional spectra. Its positioning is strategic, bridging less engaged or neutral states to those involving higher emotional and cognitive investments, thereby playing a pivotal role in the progression towards more intensely positive states.}
\label{tab:emotion_spectrums}
\vspace{-.25in}
\end{table}

\begin{comment}
\begin{table}[ht!]
\centering
\begin{footnotesize}
\begin{tabular}{lllllll}
\toprule
\textbf{-1.0} & \textbf{-0.6} & \textbf{-0.3} & \textbf{+0.3} & \textbf{+0.6} & \textbf{+1.0} \\
\toprule \midrule
Terror & Fear & Anxiety & Boldness & Courage & Heroism \\
(\textit{Horror}) & \textit{Apprehension} & \textit{Nervousness} & \textit{Daring} & \textit{Bravery} & \textit{Valor} \\
\toprule
Despair & Sadness & Melancholy & Contentment & Happiness & Joy \\
(\textit{Hopelessness}) & \textit{Gloom} & \textit{Sorrow} & \textit{Satisfaction} & \textit{Cheer} & \textit{Elation} \\
\toprule
Rage & Anger & Irritation & Composure & Peacefulness & Tranquility \\
(\textit{Fury}) & \textit{Ire} & \textit{Annoyance} & \textit{Steadiness} & \textit{Calmness} & \textit{Stillness} \\
\toprule
Shock & Surprise & Startle & Expectancy & Preparedness & Anticipation \\
(\textit{Dismay}) & \textit{Astonishment} & \textit{Alarm} & \textit{Readiness} & \textit{Proactiveness} & \textit{Expectation} \\
\toprule
Revulsion & Disgust & Distaste & Appreciation & Respect & Admiration \\
(\textit{Repugnance}) & \textit{Loathing} & \textit{Dislike} & \textit{Empathetic} & \textit{Esteem} & \textit{Compassion} \\
\toprule
Paranoia & Distrust & Suspicion & Confidence & Trust & Faith \\
(\textit{Mistrust}) &\textit{Wariness} & \textit{Cautiousness} & \textit{Assurance} & \textit{Reliance} & \textit{Conviction} \\
\hline \bottomrule
\end{tabular}
\end{footnotesize}
\vspace{.1in}
\caption{Spectrum of Emotional Dynamics: Each row includes synonyms that enhance understanding of basic emotions, allowing for simple algebraic operations such as negation or scaling on the same row to adjust emotional intensity. Neutral emotion
of each row are: Calm Alertness, Equanimity, Tolerance, Mild Interest, Acceptance, and Prudence.}
\label{tab:emotion_spectrums}
\end{table}
\end{comment}


==> TableLingEmotionColor.tex <==
\begin{table}[th!]
\vspace{-.1in}
\begin{footnotesize}
\centering
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Emotion (Int.)} & \textbf{Despair} & \textbf{Longing} & \textbf{Wishful.} & \textbf{Neutral} & \textbf{Hopeful} & \textbf{Content.} & \textbf{Joy} \\
\textbf{} & \textbf{(-1)} & \textbf{(-0.6)} & \textbf{(-0.3)} & \textbf{(0)} & \textbf{(+0.3)} & \textbf{(+0.6)} & \textbf{(+1)} \\ \midrule
Love (+1)             & \cellcolor{color4}19                   & -                      & \cellcolor{color6}54                         & \cellcolor{color6}43                  & -                      & \cellcolor{color6}53                         & \cellcolor{color6}43              \\
Admiration (+1)       & \cellcolor{color3}4                    & -                      & \cellcolor{color3}6                          & \cellcolor{color5}14                  & -                      & -                          & \cellcolor{color3}6               \\
Anticipation (+1)     & -                    & -                      & -                          & -                   & -                      & -                          & \cellcolor{color4}8               \\
Affection (+1)        & -                    & -                      & -                          & -                   & -                      & -                          & \cellcolor{color3}7               \\
Joy (+1)              & \cellcolor{color4}10                   & \cellcolor{color3}7                      & \cellcolor{color6}35                         & -                   & \cellcolor{color6}28                     & \cellcolor{color2}4                          & \cellcolor{color5}15              \\
Content. (+0.6)    & -                    & \cellcolor{color2}4                      & \cellcolor{color3}5                          & -                   & \cellcolor{color6}30                     & \cellcolor{color5}18                         & \cellcolor{color3}5               \\
Happiness (+0.6)      & \cellcolor{color4}10                   & \cellcolor{color3}7                      & \cellcolor{color4}10                         & -                   & \cellcolor{color6}29                     & -                          & \cellcolor{color3}7               \\
Trust (+0.6)          & -                    & -                      & -                          & \cellcolor{color4}11                  & -                      & -                          & -               \\
Hope (+0.3)           & -                    & -                      & \cellcolor{color6}26                         & -                   & -                      & -                          & -               \\
Boldness (+0.3)       & \cellcolor{color3}3                    & -                      & -                          & \cellcolor{color4}8                   & -                      & -                          & -               \\
Calm (+0.3)           & -                    & -                      & -                          & \cellcolor{color4}10                  & -                      & -                          & -               \\
Longing (-0.6)        & -                    & \cellcolor{color6}20                     & \cellcolor{color5}12                         & \cellcolor{color2}4                   & -                      & -                          & -               \\
Anxiety (-0.3)        & \cellcolor{color3}4                    & \cellcolor{color3}4                      & -                          & -                   & \cellcolor{color2}3                      & -                          & -               \\
Fear (-0.6)           & \cellcolor{color3}7                    & \cellcolor{color3}5                      & \cellcolor{color5}12                         & \cellcolor{color2}4                   & \cellcolor{color2}3                      & \cellcolor{color2}4                          & \cellcolor{color4}8               \\
Sadness (-0.6)        & \cellcolor{color5}24                   & \cellcolor{color5}18                     & \cellcolor{color6}28                         & \cellcolor{color5}17                  & \cellcolor{color4}10                     & -                          & \cellcolor{color3}5               \\
Melancholy (-0.6)     & \cellcolor{color5}21                   & \cellcolor{color5}19                     & \cellcolor{color3}6                          & \cellcolor{color3}6                   & \cellcolor{color2}4                      & -                          & -               \\
Despair (-1)          & \cellcolor{color6}27                   & \cellcolor{color3}8                      & \cellcolor{color5}15                         & -                   & \cellcolor{color3}9                      & -                          & \cellcolor{color3}7               \\
\bottomrule
\end{tabular}
    
\end{footnotesize}
\vspace{.05in}
\caption{Sorted top emotions in articles of linguistic behaviors}
\vspace{-.2in}
\label{tab:emocolorbeh}
\end{table}





==> TableLingEmotionsGPT4.tex <==
\begin{table}[th!]
\centering
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Emotion (Int.)} & \textbf{Despair} & \textbf{Longing} & \textbf{Wishful.} & \textbf{Neutral} & \textbf{Hopeful} & \textbf{Content.} & \textbf{Joy} \\
\textbf{} & \textbf{(-1)} & \textbf{(-0.6)} & \textbf{(-0.3)} & \textbf{(0)} & \textbf{(+0.3)} & \textbf{(+0.6)} & \textbf{(+1)} \\ \midrule
Joy (+1)              & \cellcolor{color1}  & \cellcolor{color2} & \cellcolor{color3} & \cellcolor{color4} & \cellcolor{color5} & \cellcolor{color6} & \cellcolor{color6} \\
Content. (+0.6)    & \cellcolor{color1}  & \cellcolor{color2}  & \cellcolor{color3}  & \cellcolor{color4} & \cellcolor{color5} & \cellcolor{color6} & \cellcolor{color5} \\
Happiness (+0.3)      & \cellcolor{color1}  & \cellcolor{color2}  & \cellcolor{color3}  & \cellcolor{color4}  & \cellcolor{color5} & \cellcolor{color5} & \cellcolor{color4} \\
Love (+0.6)           & \cellcolor{color1}  & \cellcolor{color2}  & \cellcolor{color3} & \cellcolor{color4} & \cellcolor{color5} & \cellcolor{color6} & \cellcolor{color6} \\
Calm (0)              & \cellcolor{color1}  & \cellcolor{color1}  & \cellcolor{color2}  & \cellcolor{color3}  & \cellcolor{color4}  & \cellcolor{color5}  & \cellcolor{color4}  \\
Trust (+0.3)          & \cellcolor{color1}  & \cellcolor{color1}  & \cellcolor{color2}  & \cellcolor{color3}  & \cellcolor{color4} & \cellcolor{color4} & \cellcolor{color3} \\
Hope (+0.3)           & \cellcolor{color1}  & \cellcolor{color2}  & \cellcolor{color3}  & \cellcolor{color4} & \cellcolor{color5} & \cellcolor{color5} & \cellcolor{color4} \\
Fear (-0.6)           & \cellcolor{color2} & \cellcolor{color3} & \cellcolor{color4} & \cellcolor{color5} & \cellcolor{color4} & \cellcolor{color3} & \cellcolor{color2} \\
Anxiety (-0.3)        & \cellcolor{color3} & \cellcolor{color4} & \cellcolor{color5} & \cellcolor{color6} & \cellcolor{color5} & \cellcolor{color4} & \cellcolor{color3} \\
Sadness (-0.6)        & \cellcolor{color4} & \cellcolor{color5} & \cellcolor{color6} & \cellcolor{color6} & \cellcolor{color5} & \cellcolor{color4} & \cellcolor{color3} \\
Despair (-1)          & \cellcolor{color5} & \cellcolor{color6} & \cellcolor{color6} & \cellcolor{color5} & \cellcolor{color4} & \cellcolor{color3} & \cellcolor{color2} \\
\bottomrule
\end{tabular}
\vspace{.1in}
\caption{Frequency of emotions of diff. linguistic behaviors, colored by intensity, generated by GPT-4}
\label{tab:emotions_behavior_askGPT4}
\end{table}



==> TableLoveLetter.tex <==
Tables~\ref{tab:love_speech_spectrum} and~\ref{tab:neutral_speech_spectrum} examine linguistic behaviors 
across a spectrum in two contexts: 
{\em Love Letter} and {\em Neutral Speech}, correlating specific emotions with distinct behavioral expressions.
These two tables are generated by prompting GPT-4. It is evident that while the spectrum of linguistic
behaviors appear to be reasonable, the emotions that GPT-4 use for depicting behaviors may not appear
on in Table~\ref{tab:emotion_spectrums}. Our second pilot study in Section~\ref{sec:exp} will 
compare the quality of mappings
between GPT-4's directly responses and our self-supervised learning pipeline.
({\color{red}Please specify the performance metrics.})

%Note that in psychological terms, behaviors and emotions are often interrelated, which can cause the terms to overlap. In emotional expression, behaviors such as writing a love letter or expressing despair can be driven by underlying emotions. However, those behaviors themselves can also evoke or be characterized by specific emotions, blurring the lines between what is considered a behavior and what is an emotion.

\begin{table}[ht!]
\centering
\begin{footnotesize}
\begin{tabular}{lll}
\toprule
\textbf{Int.} & \textbf{Description} & \textbf{Emotions} \\
\toprule
\hline
-1.0 & Despair: Expresses profound sadness, feeling of loss & Despair, Grief \\
\hline
-0.6 & Longing: Strong yearning or pining for the loved one & Sadness, Longing \\
\hline
-0.3 & Wistfulness: Mild longing mixed with nostalgia & Melancholy, Wistfulness \\
\hline
0.0 & Neutral: Communicates feelings straightforwardly & Serenity, Neutral \\
\hline
0.3 & Hopeful: Optimistic about the relationship’s future & Anticipation, Hopefulness \\
\hline
0.6 & Contentment: Satisfaction and joy in relationship & Contentment, Pleasure \\
\hline
1.0 & Joyful Affection: Intense happiness and love & Joy, Elation \\
\hline
\bottomrule
\end{tabular}
\end{footnotesize}
\vspace{.1in}
\caption{Love Letter Spectrum}
\label{tab:love_speech_spectrum}
\end{table}


\begin{table}[ht!]
\centering
\begin{footnotesize}
\begin{tabular}{lll}
\toprule
\textbf{Int.} & \textbf{Description} & \textbf{Emotions} \\
\toprule
\hline
-1.0 & Hate Speech: Overtly aggressive, derogatory, violent & Rage, Disgust \\
\hline
-0.6 & Hostile Remarks: Explicitly prejudiced or damaging & Anger, Contempt \\
\hline
-0.3 & Biased Remarks: Subtle biases, possibly unintentional & Annoyance, Discomfort \\
\hline
0.0 & Neutral: Factual, unbiased communication & Neutrality \\
\hline
0.3 & Polite Mention: Respectful, considerate language & Courtesy, Respect \\
\hline
0.6 & Inclusive Language: Recognizes and respects diversity & Acceptance, Empathy \\
\hline
1.0 & Advocative Speech: Promotes understanding, equality & Compassion, Admiration \\
\hline
\bottomrule
\end{tabular}
\end{footnotesize}
\vspace{.1in}
\caption{Neutral Speech Spectrum}
\label{tab:neutral_speech_spectrum}
\end{table}


==> TraditionalEmotionWheels.tex <==
\begin{figure}[ht!]
%\vspace{-.1in}
    \centering
    \subfloat[Plutchik’s Wheel of Emotions \cite{plutchik1980general}]{%
        \includegraphics[width=0.43\textwidth]{PlutchikWheel-of-Emotions.jpg}
        \label{fig:Plutchik}
    }
    \hspace{.05in}
    \subfloat[Adopted from Geneva Wheel \cite{GenevaEmotionWheelRobots2018}]{%
        \includegraphics[width=0.48\textwidth]{The-Emotion-Wheel-and-Our-Associated-Questionnaire-Notes-both-adapted-from-3.png}
        \label{fig:Geneva}
    }
    \caption{Comparative display of emotional models. These models include only the “basic” emotions. Complex emotions can be modeled with basic emotions.}
    \label{fig:emotion_models}
\end{figure}

